Learning and Tuning Meta-heuristics in Plan Space Planning

In recent years, the planning community has observed that techniques for learning heuristic functions have yielded improvements in performance. One approach is to use offline learning to learn predictive models from existing heuristics in a domain dependent manner. These learned models are deployed as new heuristic functions. The learned models can in turn be tuned online using a domain independent error correction approach to further enhance their informativeness. The online tuning approach is domain independent but instance specific, and contributes to improved performance for individual instances as planning proceeds. Consequently it is more effective in larger problems. In this paper, we mention two approaches applicable in Partial Order Causal Link (POCL) Planning that is also known as Plan Space Planning. First, we endeavor to enhance the performance of a POCL planner by giving an algorithm for supervised learning. Second, we then discuss an online error minimization approach in POCL framework to minimize the step-error associated with the offline learned models thus enhancing their informativeness. Our evaluation shows that the learning approaches scale up the performance of the planner over standard benchmarks, specially for larger problems.

==> accuracy.tex <==
%
%
%
%
\begin{tabular}
{
	@{}
	l 		  @{~~} %@{\quad} %@{\qquad }  
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{}
}
\toprule
%
%
\multirow{2}{*}{{RT}}
& \multicolumn{2}{@{}c@{}}{\normalfont{$h_{{add}}$}}
& \multicolumn{2}{@{}c@{}}{\normalfont{\emph{w. effort}}}%{{with \textit{effort}}}	
& \multicolumn{2}{@{}c@{}}{\normalfont{$h_{{add}}^{{r}}$}}
& \multicolumn{2}{@{}c@{}}{\normalfont{\emph{w. effort}}} %{{with \textit{effort}}} }
\\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(){8-9}
% 				
%
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu} 
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu} 
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu}
 	& \normalfont{\emph{corr}} 
 	& \normalfont{\sc cpu} 
 	\\ \cmidrule(r){1-1} \cmidrule(r){2-3} \cmidrule(r){3-3}\cmidrule(r){4-5}
 							\cmidrule(lr){5-5}\cmidrule(r){6-7} \cmidrule(lr){7-7} \cmidrule(r){8-9} \cmidrule(l){9-9}
%																										
%
LR		& 	0.98 &	17 	& 0.92 & 23 	&  0.83	& 24 	& 	0.89 &  	22 \\ 
LMS 	&	0.97 & 	203 & 0.92 & 233 & 0.83 	& 138 	& 	0.93 & 	149 \\
MLP 	& 	0.98 & 	540	& 0.93 & 613 & 0.76 	& 483 	& 	0.92 & 	490	\\
M5Rule 	& 	0.98 & 	67	& 0.98 & 103 & 0.98 	& 75	& 	0.88 &	105	\\
M5P 	& 	0.98 & 	50 	& 0.94 & 70 	& 0.98 	& 42 	& 	0.87 & 	38  \\
\bottomrule
\end{tabular}%
%
%
%

==> corr-icaps-2016/accuracy.tex <==
%
%
%
%
\begin{tabular}
{
	@{}
	l 		  @{~~} %@{\quad} %@{\qquad }  
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{\quad} 
	>{\small\tt} r @{~~} %@{\quad} 
	>{\small\tt} r @{}
}
\toprule
%
%
\multirow{2}{*}{{RT}}
& \multicolumn{2}{@{}c@{}}{\normalfont{$h_{{add}}$}}
& \multicolumn{2}{@{}c@{}}{\normalfont{\emph{w. effort}}}%{{with \textit{effort}}}	
& \multicolumn{2}{@{}c@{}}{\normalfont{$h_{{add}}^{{r}}$}}
& \multicolumn{2}{@{}c@{}}{\normalfont{\emph{w. effort}}} %{{with \textit{effort}}} }
\\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(){8-9}
% 				
%
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu} 
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu} 
	& \normalfont{\emph{corr}} 
	& \normalfont{\sc cpu}
 	& \normalfont{\emph{corr}} 
 	& \normalfont{\sc cpu} 
 	\\ \cmidrule(r){1-1} \cmidrule(r){2-3} \cmidrule(r){3-3}\cmidrule(r){4-5}
 							\cmidrule(lr){5-5}\cmidrule(r){6-7} \cmidrule(lr){7-7} \cmidrule(r){8-9} \cmidrule(l){9-9}
%																										
%
LR		& 	0.98 &	17 	& 0.92 & 23 	&  0.83	& 24 	& 	0.89 &  	22 \\ 
LMS 	&	0.97 & 	203 & 0.92 & 233 & 0.83 	& 138 	& 	0.93 & 	149 \\
MLP 	& 	0.98 & 	540	& 0.93 & 613 & 0.76 	& 483 	& 	0.92 & 	490	\\
M5Rule 	& 	0.98 & 	67	& 0.98 & 103 & 0.98 	& 75	& 	0.88 &	105	\\
M5P 	& 	0.98 & 	50 	& 0.94 & 70 	& 0.98 	& 42 	& 	0.87 & 	38  \\
\bottomrule
\end{tabular}%
%
%
%

==> corr-icaps-2016/gen-vis-time.tex <==
%
%
%
\begin{tabular}
%		
{
%
	@{}
				l
				>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad}  	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r
	@{}				
%
}
%
\toprule
%
	\multirow{2}{*}{Domain} & 
	\multicolumn{3}{c}{$h_{{add}}$} & 
	\multicolumn{3}{c}{\sc wef} & 
	\multicolumn{3}{c}{$h_{{add}}^r$} & 
	\multicolumn{3}{c}{\sc  wef} & 
	\multicolumn{3}{c}{$h_{{add}}$-\sc l } & 
	\multicolumn{3}{c}{$h_{{add}}\text{-\sc le}$} & 
	\multicolumn{3}{c}{\sc wef-l} & 
	\multicolumn{3}{c}{\sc wef-{le}} 
		\\ 	\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} \cmidrule(r){17-19}
			\cmidrule(r){20-22} \cmidrule(){23-25} 
	%
 	& 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} &
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} 
		\\ 		\cmidrule(r){1-1} \cmidrule(r){2-4} \cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(r){5-7}\cmidrule(lr){6-6}
				\cmidrule(lr){7-7}\cmidrule(r){8-10}\cmidrule(lr){9-9}\cmidrule(lr){10-10}\cmidrule(r){11-13} \cmidrule(lr){12-12}
				\cmidrule(lr){13-13}
				\cmidrule(r){14-16}\cmidrule(lr){15-15}\cmidrule(lr){16-16}\cmidrule(r){17-19}\cmidrule(lr){18-18}\cmidrule(lr){19-19}
				\cmidrule(r){20-22}
				\cmidrule(lr){21-21}\cmidrule(lr){22-22}\cmidrule(r){23-25}\cmidrule(lr){24-24}\cmidrule(l){25-25}
		%
		Gripper& 191 & 51 & 10 & 51 & 27 & 3.4 & 93 & 75 & 2.1 & 93 & 75 & 2.1
			 	& 38 & 17 & 1.4 & 37 & 17 & 2.3 & 37 & 17 & 2.3 &
			 	37 & 17 & 2.2 \\
		Rovers-3& 16 & 10 & 0.7 & 36 & 22 & 1.5 & 8 & 6 & 0.5 & 4 & 3 & 0.3
			 	& 19 & 7 & 0.9 & 19 & 9 & 10 & 19 & 9 & 10 & 19 & 9 & 10 \\ 
		Rovers -5& 70 & 32 & 3 & 67 & 38 & 5.2 & 96 & 51 & 12 & 34 & 26 & 11 &
			 	49 & 32 & 10 & 51 & 36 & 11 & 66 & 45 & 13 & 51 & 36 & 7 \\
		%
		%
\midrule
		%
		%
		\multirow{1}{*}{Domain} & 
		\multicolumn{3}{c}{$h_{{add}}$} & 
		\multicolumn{3}{c}{\sc wef} & 
		\multicolumn{3}{c}{$h_{{add}}^r$} & 
		\multicolumn{3}{c}{\sc wef} & 
		\multicolumn{3}{c}{$h_{{add}}^r$-\sc l}   & 
		\multicolumn{3}{c}{$h_{{add}}^r\text{-\sc le}$} & 
		\multicolumn{3}{c}{\sc wef-l}  &   							 
  		\multicolumn{3}{c}{\sc wef-{le}} 
			\\ 		\cmidrule(r){1-1} \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} 
					\cmidrule(r){14-16} \cmidrule(r){17-19} \cmidrule(r){20-22} \cmidrule(l){23-25} 
		%			 
		Logistics-1 & 89 & 9.5 & 100 & 0.4 & 0.2 & 0 & 64 & 12 & 64 & 1.9 & 0.6 & 46 &
				3 & 0.4 & 44 & 3 & 0.4 & 64 & 1.4 & 0.3 & 26 & 3 & 0.4 & 65 \\		 
		%
		%
		Elevator& 81 & 5.4 & 2 & 0.3 & 0.2 & 0 & 50 & 5 & 4 & 30 & 8 & 3 &
				12 & 1 & 0.6 & 12 & 1 & 0.6 & 12 & 1 & 0.6 &12 & 1 & 0.6  \\ 
		%
		Logistics-2 & 2 & 0.9 & 0.2 & 10 & 7 & 0.7 & 2.6 & 1.2 & 0.6 & 3 & 1.8 & 1 &
				0.6 & 0.2 & 0.1 & 0.6 & 0.2 & 0.1& 0.6 & 0.2 & 0.1& 0.6 & 0.2 & 0.1 \\
		%
		Zenotravel & 93 & 15 & 0.9 & 98 & 14 & 1 & 162 & 19 & 4 & 66 & 6 & 2&
				80 & 5 & 2.5 & 87 & 6.8 & 0.2 & 80 &4.5 & 2.9 & 88 & 7 & 2 \\				
%
\bottomrule			 
%
\end{tabular}
%
%

==> corr-icaps-2016/ipc-4.tex <==
\begin{tabular}{l @{\quad} >{\tt}c @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad}>{\tt}r @{\quad}
>{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r }%{|l|c|r| r r r |r| r r r |}
%
%
	\toprule
%
	\multirow{2}{*}{ \makecell{Domain \\ (IPC-4)} }  &
	%\multirow{2}{*}{ \normalfont Ins} &
	\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=r]{90}{\normalfont ~Ins}}} &
 	\multicolumn{4}{c}{$h_{{add}}^{{a}}$ with effort} & 		
	\multicolumn{4}{c}{$h_{{add}}$ with effort} 	\\ \cmidrule(r){3-6} \cmidrule{7-10}
	%
 	& & \multirow{1}{*}{\normalfont S} &
 	{\normalfont Gen} & {\normalfont Vis} & {\normalfont CPU} & \multirow{1}{*}{\normalfont S} &
 	{\normalfont Gen} & {\normalfont Vis} & {\normalfont CPU} \\ 
 	%
 	%
	%
	\cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){6-6}
		\cmidrule(r){7-10} \cmidrule(r){8-8} \cmidrule(r){9-10} \cmidrule(){10-10	}
	%
	%
	%	IPC-4
	Pipesworld-noTankage	&20	&{6}	&	8.3K	&	1.9K	&89		&5	&	8.1K	&1.4K	&109
	\\
	Pipesworld-tankage		&	20	& {3}	& {31K}	& {2.6K}	& {773}	&3	&	81K	&	6.9K	&2.1K
	\\
	Satellite	&	36	&	{24}	&	{96K}&	{4.1K}	&	{3.5K}	&2	&1.1K	&361	&2 
	\\ \bottomrule	
	%
	%
	%
\end{tabular}

==> corr-icaps-2016/makespan-icaps-1-2016.tex <==
%
%
%
\begin{tabular}
%		
{@{}l || r r | r r || r r | r r@{}}
%
\hline
%
%	\multirow{1}{*}{\textbf{Domain}} &
%	\multicolumn{8}{c|}{\textbf{POCL Heuristics}} 
%	\\ \cline{2-9}
%
%	&
%	\multicolumn{4}{c||}{\textbf{State-of-the-art}} &
%	\multicolumn{4}{c|}{\textbf{Via learning approaches}} 
%	\\ \cline{2-9} 
	%
	\multirow{1}{*}{\textbf{Domain}} &
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{l}}$} & 
	\multicolumn{1}{c@{}}{$h_{{add,w}}^{{l,e}}$} 
%	
%
%
	\\ 	\hline \hline
%	
	Gripper-1 	&16.0	&9.8	&0.5	&0.5		&\textbf{20.0}  &\textbf{20.0}	&\textbf{20.0}	&\textbf{20.0} \\
	%
	Rovers-3 	&\textbf{17.9}	&15.5	&17.8	&15.8		&17.4		&{17.7} 	&17.4		&{17.7} \\
	%
	Rovers-5	&26.1	&24.2	&28.4	&26.5		&\textbf{30.5}		&${}^{\text{\small +}}$29.8	
																							&${}^{\text{\small +}}$27.6	&\textbf{30.5} \\
	%
	%\cline {3-18} 			 
	\hline
	%
    &
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{r,l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{r,l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l}}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l,e}}$}  \\	
	%
	\hline
	%
	%
	Logistics-1	&21.8	&0.9	&25.2	&20.8	
							&${}^{\text{\small +}}$30.4	&${}^{\text{\small +}}$30.4	&17.6	&\textbf{30.5} \\
	%
	Elevator-2		&147.1	&11.7	&\textbf{149.1}	&50.5		&	\textbf{149.1}	
							&146.8		&\textbf{149.1} &	146.8	\\
	%							
	Logistics-2	&26.3	&7.0	&33.0	&19.3	&${}^{\text{\small +}}$33.5	&\textbf{35.4}	 
							&${}^{\text{\small +}}$33.4	&\textbf{35.4}   \\
	%
	Zenotravel-3	&3.7	&2.7	&7.5	&7.7		&${}^{\text{\small +}}$12.1
									&\textbf{13.5}		&${}^{\text{\small +}}$12.1		&\textbf{13.5} \\
	%
	%
	\hline 
%
\end{tabular}
%
%

==> corr-icaps-2016/plan-score-icaps-1-2016.tex <==
%
%
%
\begin{tabular}
%		
{ @{} l || r r | r r || r r | r r || r r r r || r r r r ||r @{}}
%
\hline
%
	\multirow{3}{*}{\textbf{Domain}} &
	\multicolumn{8}{c||}{\textbf{POCL Heuristics}} &
	\multicolumn{8}{c||}{\textbf{Evaluation using Fast Downward (FD)}} &
	\multirow{3}{*}{\textbf{LAMA}} 
	\\ \cline{2-17}
%
	&
	\multicolumn{4}{c||}{\textbf{State-of-the-art}} &
	\multicolumn{4}{c||}{\textbf{Via learning approaches}} &
	\multicolumn{4}{c||}{\textbf{Lazy}} &
	\multicolumn{4}{c||}{\textbf{Eager}} & 
	\\ \cline{2-17} 
	%
	&
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{l}}$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{{l,e}}$} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &	
%
%
	\\ 	\hline \hline
%	
	Gripper-1 	&16.0	&14.9	&0.7	&0.7		&\textbf{20.0}		&\textbf{20.0}		&\textbf{20.0}		&\textbf{20.0}		
						&15.45 		&14.9			&15.5 		&15.5		
						&15.5		&14.9			&15.5 	&15.5	&\textbf{20.0} \\
	%
	Rovers-3 	&17.3	&16.2	&18.1	&16.9		&17.8		&${}^{\text{\small +}}$18.6	&17.8 &${}^{\text{\small +}}$18.6
						&17.1	&15.9	&12.5	&18.8		&18.1		&16.9		&13.9	&19.0		&\textbf{19.8}	 \\
	%
	Rovers-5	&25.7		&26.3		&28.0	&30.2		&${}^{\text{\small +}}$33.1	&${}^{\text{\small +}}$36.3	&30.1		
						&${}^{\text{\small +}}$33.6	&20.8		&23.4	&13.5		&26.0		&22.7	&27.3	&15.7	&28.3		
						&\textbf{39.8} \\
%
	%\cline {3-18} 			 
\hline
	%
    &
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{r,l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{r,l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l}}$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{{r,l,e}}$} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} & \\ 
	%
	\hline
	% \cline{3-18}
	%
	Logistics-1	&24.3	&0.8	&31.2	&26.1	
							&${}^{\text{\small +}}$31.2	&${}^{\text{\small +}}$31.2	&20.9		&\textbf{32.0}
							&23.7		&30.3		&19.7		&27.4		&27.0			&30.8		&15.1		&24.6		&30.8 \\
	%
	Elevator-2		&142.8	&11.8	&144.9	&49.7		&142.7	
							&${}^{\text{\small +}}$144.9		&142.7
							&${}^{\text{\small +}}$144.9										
							&117.1	&112.0	&117.1	&116.9
							&144.1	&136.0	&144.2	&141.0	&\textbf{148.2}	\\
	%							
	Logistics-2	&33.8		&10.7		&34.9		&30.7		&\textbf{38.1}		&${}^{\text{\small +}}$36.3	
																			&\textbf{38.1}		&${}^{\text{\small +}}$36.3
							&33.72		&29.5		&32.4		&33.3		&34.1		&30		&33.7		&35.6			&37.8	\\
	%
	Zenotravel-3	&4.6		&3.7		&8.5		&8.8		&${}^{\text{\small +}}$13.5	&${}^{\text{\small +}}$13.7	
							&${}^{\text{\small +}}$13.5 	&${}^{\text{\small +}}$13.7
							&17.3 	&17.7		&14.7 	&18.6	
							&18.1		&14.3 	&16		&18.8	&\textbf{19.2} \\
	%
	%
	\hline \hline
	\multicolumn{1}{@{}c||}{\textbf{Time Score}}
							&204.4		&76.5		&197.7	 	&148.6		&${}^{\text{\small +}}$272.9		&${}^{\text{\small +}}$260.8
							&${}^{\text{\small +}}$258.6		&${}^{\text{\small +}}$264.3		&255.6	
							&\textbf{280.0}		&228.0		&233.8		&259.6		&271.3		&223.0		&222.5		&137 \\					
%
%														
\hline			 
%
\end{tabular}
%
%

==> corr-icaps-2016/plan-visited-icaps-1-2016.tex <==
%
%
%
\begin{tabular}
%		
{@{} l || r r | r r || r r | r r @{}}
%
\hline
%
%	\multirow{3}{*}{\textbf{Domain}} &
%	\multicolumn{8}{c|}{\textbf{POCL Heuristics}} 
%	\\ \cline{2-9}
%
	\multirow{2}{*}{\textbf{Domain}} &
	\multicolumn{4}{c||}{\textbf{State-of-the-art}} &
	\multicolumn{4}{c}{\textbf{Via learning approaches}} 
	\\ \cline{2-9} 
	%
	&
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{l}}$} & 
	\multicolumn{1}{c@{}}{$h_{{add,w}}^{{l,e}}$} 
%	
%
%
	\\ 	\hline \hline
%	
	Gripper-1 	&7.0	&14.0	&0.0	&0.0	&${}^{\text{\small +}}$18.0  &\textbf{19.7}	&${}^{\text{\small +}}$18.0	&\textbf{19.7} \\
	%
	Rovers-3 	&8.6	&8.3	&12.6 	&\textbf{19.0}		&13.3	&13.6 	&13.3	&13.6 \\
	%
	Rovers-5	&8.2	&14.7	&13.5	&30.9		&\textbf{31.4}		&\textbf{31.4}		&24.7 &\textbf{31.4}	\\
%
	%\cline {3-18} 			 
	\hline
	%
    &
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{r,l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{r,l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l}}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l,e}}$} \\	
	%
	\hline
	%
	%
	Logistics-1	&5.1	&0.6	&16.5	&21.6	
							&\textbf{29.9}		&\textbf{29.9}		&{20.7}	&\textbf{29.9} \\
	%
	Elevator-2		&41.4	&8.2	&58.9	&39.7		&\textbf{145.0} 		
														&${}^{\text{\small +}}$135.0	&\textbf{145.0}	&${}^{\text{\small +}}$135.0	\\
	%							
	Logistics-2	&24.5	&6.5	&23.4	&26.7		&${}^{\text{\small +}}$33.4	
														&\textbf{35.3}	 &${}^{\text{\small +}}$33.4	&\textbf{35.3}   \\
	%
	Zenotravel-3	&0.0	&1.0	&2.4	&7.7 	&7.4	&\textbf{11.07}	&7.4	&\textbf{11.07} \\
	%
	%
	\hline 
%
\end{tabular}
%
%

==> corr-icaps-2016/problems-coverage-icaps-1-2016.tex <==
%
%
%
\begin{tabular}
%		
{ @{} l | r || r r | r r || r r | r r || r r r r || r r r r ||r @{}}
%
\hline
%
	\multirow{3}{*}{\textbf{Domain}} &
	\multirow{3}{*}{\textbf{\#}} &
	\multicolumn{8}{c||}{\textbf{POCL Heuristics}} &
	\multicolumn{8}{c||}{\textbf{Evaluation using Fast Downward (FD)}} &
	\multirow{3}{*}{\textbf{LAMA}} 
	\\ \cline{3-18}
%
	&
	&
	\multicolumn{4}{c||}{\textbf{State-of-the-art}} &
	\multicolumn{4}{c||}{\textbf{Via learning approaches}} &
	\multicolumn{4}{c||}{\textbf{Lazy}} &
	\multicolumn{4}{c||}{\textbf{Eager}} &
	\\ \cline{3-18} 
	%
	 & &
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{l}}$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{{l,e}}$} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &	
%
%
	\\ 	\hline \hline
%	
	Gripper-1 	&20		&16		&\textbf{20}		&1		&1		&\textbf{20}		&\textbf{20}	&\textbf{20}		&\textbf{20}		
						&\textbf{20} 	&\textbf{20}		&\textbf{20} 	&\textbf{20}		
						&\textbf{20} 	&\textbf{20}		&\textbf{20} 	&\textbf{20}		&\textbf{20} \\
	%
	Rovers-3 	&20		&19		&19		&\textbf{20}		&\textbf{20}		&\textbf{20}		&\textbf{20}		&\textbf{20}		
																														&\textbf{20}																	
						&18		&17		&14		&\textbf{20}		&19		&18		&15		&\textbf{20}		&\textbf{20}	 \\
	%
	Rovers-5	&40		&28		&31		&32		&36		&${}^{\text{\small +}}$39		&${}^{\text{\small +}}$39	
						&${}^{\text{\small +}}$36		&${}^{\text{\small +}}$39															
						&22		&25		&15		&28		&24		&29		&17		&30		&\textbf{40} \\
%
	\cline {1-19} 			 
%
    &
	&
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c|}{$h_{{add,w}}$} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{r}$} & 
	\multicolumn{1}{c}{$h_{{add}}^{{r,l}}$} & 
	\multicolumn{1}{c|}{$h_{{add}}^{r,l,e}$} & 
	\multicolumn{1}{c}{$h_{{add,w}}^{{r,l}}$} & 
	\multicolumn{1}{c||}{$h_{{add,w}}^{{r,l,e}}$} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} &
	%
	\multicolumn{1}{c}{FF} & 
	\multicolumn{1}{c}{CEA} &
	\multicolumn{1}{c}{LM-Cut} &
	\multicolumn{1}{c||}{MHFS} & \\ 
	%
	% \cline{3-18}
	\hline
	%
	Logistics-1	&35 	&25		&1		&32		&28		&${}^{\text{\small +}}$32		&${}^{\text{\small +}}$32 	&22
							&${}^{\text{\small +}}$32	
							&25		&34		&21		&28		&28		&34		&16		&25		&\textbf{35} \\
	%
	Elevator-2		&150	&148	&14		&\textbf{150}	&58		&\textbf{150}	&\textbf{150}	&\textbf{150}	&\textbf{150}										
							&\textbf{150}	&\textbf{150}	&\textbf{150}	&\textbf{150}
							&\textbf{150}	&\textbf{150}	&\textbf{150}	&\textbf{150}	&\textbf{150}	\\
	%							
	Logistics-2	&40		&36		&12		&36		&34		&\textbf{40}	&\textbf{40}	&\textbf{40}	&\textbf{40}
							&36		&36		&35		&36		&36		&36		&36		&36		&\textbf{40}	\\
	%
	Zenotravel-3	&20		&5		&4		&9		&10		&${}^{\text{\small +}}$16		&${}^{\text{\small +}}$16
							&${}^{\text{\small +}}$16		&${}^{\text{\small +}}$16
							&\textbf{20}		&\textbf{20} 	&17		&\textbf{20}	
							&\textbf{20}		&\textbf{20} 	&16		&\textbf{20}	&\textbf{20} \\
%
%														
\hline			 
%
\end{tabular}
%
%

==> corr-icaps-2016/problems-coverage-icaps-2016.tex <==
%
%
%
\begin{tabular}
%		
{ l | r r r r r r r r r r r r r r r r r}
%
\toprule
%
	\multirow{2}{*}{Domain} &
	\multicolumn{8}{c}{POCL Heuristics} &
	\multicolumn{5}{c}{Lazy} &
	\multicolumn{5}{c}{Eager}
	\\ \cmidrule{2-19}
	%
	 & 
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c}{\sc wef} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c}{\sc  wef} & 
	\multicolumn{1}{c}{$h_{{add}}$-\sc l } & 
	\multicolumn{1}{c}{$h_{{add}}\text{-\sc le}$} & 
	\multicolumn{1}{c}{\sc wef-l} & 
	\multicolumn{1}{c}{\sc wef-{le}} &
	%
	\multicolumn{1}{c}{\sc ff} & 
	\multicolumn{1}{c}{\sc cea} &
	\multicolumn{1}{c}{\sc lmcut} &
	\multicolumn{1}{c}{\sc mhfs} &
	\multicolumn{1}{c}{\sc lama} &
	%
	\multicolumn{1}{c}{\sc ff} &
	\multicolumn{1}{c}{\sc cea} &
	\multicolumn{1}{c}{\sc lmcut} &
	\multicolumn{1}{c}{\sc mhfs} &
	\multicolumn{1}{c}{\sc lama}	
%
%
	\\ 	\midrule
%	
\bottomrule			 
%
\end{tabular}
%
%

==> corr-icaps-2016/solved-instances.tex <==
%
%
\begin{tabular}
%
{ 
	@{}
	l 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad}	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad}  	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{}
}
%
%
\toprule
	\multirow{2}{*}{Domain (n)} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}$} & 
	\multicolumn{2}{@{}c@{}}{\sc wef} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}^r$ } & 
	\multicolumn{2}{@{}c@{}}{\sc wef} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}\text{-}\text{\sc l}$ } &
  	\multicolumn{2}{@{}c@{}}{$h_{\text{add}}\text{-}{\text{\sc le}}$} & 
  	\multicolumn{2}{@{}c@{}}{\sc wef-$\text{\sc l}$}  & 
  	\multicolumn{2}{@{}c@{}}{\sc wef-{\sc le}} 
  	%
	\\ 	\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
		\cmidrule(r){10-11} \cmidrule(r){12-13}
		\cmidrule(r){14-15} \cmidrule(){16-17} 
%
%
  & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} &
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} 
 	\\ 	\cmidrule(r){1-1}  \cmidrule(r){2-3}  \cmidrule(r){3-3}  \cmidrule(r){4-5}  \cmidrule(r){5-5}  \cmidrule(r){6-7}  
 		\cmidrule(r){7-7} 	 \cmidrule(r){8-9}  \cmidrule(lr){9-9}  \cmidrule(r){10-11}  \cmidrule(r){11-11}  \cmidrule(r){12-13}
 		\cmidrule(r){13-13}  \cmidrule(r){14-15}  \cmidrule(r){15-15}  \cmidrule(r){16-17}  \cmidrule(l){17-17} 
  %  			
	Gripper (20) 	& 16 & 56 & 20 & 91 & 1 	& 15 & 1 	& 15 	& 20 & 68 & 20 & 68 & 20 & 68 & 20 & 68 \\
	Rovers-3 (20)	& 19 & 35 & 19 & 40 & 20 	& 37 & 20 	& 41 	& 20 & 37 & 20 & 37 & 20 & 37 & 20 & 37 \\
	Rovers-5 (40) 	& 28 & 48 & 31 & 65 & 32 	& 60 & 36 	& 102 	& 39 & 110 & 39 & 97 & 36 & 112 & 39 & 107 \\
  %
\bottomrule  
%			
\end{tabular}

==> corr-icaps-2016/solved-instances1.tex <==
%
%
\begin{tabular}
%
{
%	
	@{}
	l 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad}  	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{}
%
}
%
\toprule
%
%
	\multirow{2}{*}{Domain (n)} & 
	\multicolumn{2}{c}{$h_{{add}}$} & 
	\multicolumn{2}{c}{\sc wef} & 
	\multicolumn{2}{c}{$h_{{add}}^r$} & 
	\multicolumn{2}{c}{\sc wef}	& 
	\multicolumn{2}{c}{$h_{{add}}^r$-\sc l }  & 
  	\multicolumn{2}{c}{$h_{{add}}^r\text{-\sc  le}$} & 
  	\multicolumn{2}{c}{\sc wef-l} & 
  	\multicolumn{2}{c}{\sc wef-{\sc le}} 
		\\ 	\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
			\cmidrule(lr){10-11} \cmidrule(r){12-13}
			\cmidrule(r){14-15} \cmidrule(){16-17} 
%
	& 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} &
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} 
 		\\ 	\cmidrule(r){1-1}  \cmidrule(r){2-3}  \cmidrule(r){3-3}  \cmidrule(r){4-5}  \cmidrule(r){5-5}  
 			\cmidrule(r){6-7}  \cmidrule(r){7-7}
 		 	\cmidrule(r){8-9}  \cmidrule(lr){9-9}  \cmidrule(r){10-11}  \cmidrule(r){11-11}  \cmidrule(r){12-13}
 		  	\cmidrule(r){13-13}  \cmidrule(r){14-15}  \cmidrule(r){15-15}  \cmidrule(r){16-17}  \cmidrule(l){17-17}
	%  			
	Logistics-1 (35) & {25} & 102 & 1 & 36 & 32 & 90 & 28 & 73 & 32 & 90 & 32 & 90 & 22 & 70 & 32 & 90 \\
	Elevator (150) & 148 & 54 & 14 & 9 & 150 & 55 & 58 & 29 & 150 & 55 & 150 & 55  & 150 & 55 & 150 & 55 \\
	Logistics-2 (40) & 36 & 77 & 12 & 53 & 36 & 63 & 34 & 63 & 40 & 63 & 40 & 65 & 40 & 63 & 40 & 65 \\
	Zenotravel (20) & 6 & 7 & 4 & 8 & 9 & 13 & 10 & 17 & 16 & 20 & 16 & 18 & 16 & 20 & 16 & 18 \\ 
	%
	\bottomrule  			
	%
\end{tabular}
%
%

==> corr-icaps-2016/theorem-proof.tex <==
%
%
%
\subsubsection{Theorem 1.} 
\emph
{
For a given learned predictive model ($h$) and partial plan ($\pi_i$) in Figure~1 which leads to the solution plan ($\pi_{sol}$)
after certain refinement steps, the enhanced version of the predictive model ($h^e$) is,
%
%
\begin{equation}\label{eq2a:test}
		h^e(\pi_i) \ = \ h(\pi_{i}) \ + 
%				\sum_{\pi' from \{ \pi_i \rightsquigarrow \pi_{ideal} \}} \epsilon_{h(\pi')}
				\sum_{	\substack{\pi{'}~\text{{from}} \\ \pi_i \rightsquigarrow \pi_{sol}} } \epsilon_{h(\pi')}
\end{equation}
where $\pi_i$ $\rightsquigarrow$ $\pi_{sol}$ is a path in Figure~1 which captures each partial plan ($\pi'$) along 
the path between $\pi_i$ and $\pi_{sol}$.
The path includes $\pi_i$  and excludes the $\pi_{sol}$. The term $\epsilon_h$ is single-step-error associated with 
$\mathit{h}$ during refinement.
%
}
%
%
%
%
\begin{Proof} 
%
%
We use the principle of mathematical induction to prove this theorem.

\noindent $\mathit{\bold{Basis:}}$ We assume that $\pi_i$ needs only one refinement to become $\pi_{sol}$ that
would also be $\pi_i$'s best child.
%
Here, the best child always keeps the lowest estimate of requirement of new actions for its refinement among its siblings.
%
One possible refinement of $\pi_i$ is, $\pi_i \xrightarrow{R_i} \pi_{sol}$. 
Using Eq.~\eqref{eq2a:test}, we say,
%
\begin{eqnarray}\label{aeq2:test}	
		h^e(\pi_i) \ &=& \ h(\pi_{i}) \ +  \ \epsilon_{h(\pi_i)}
\end{eqnarray}	
%	
The term $\epsilon_{h(\pi_i)}$ is the single-step-error associated with \emph{h} that estimates the total effort required for
$\pi_i$ to refine it completely. For unit cost refinements (cost($R_i$) = 1), $\epsilon_{h(\pi_i)}$ is computed as,
\begin{eqnarray}\label{aeq3:test}
	\epsilon_{h(\pi_i)} = (cost(R_i) + h(\pi_{i+1})) - h(\pi_{i})
\end{eqnarray}	
%
Here, the partial plan $\pi_{i+1}$ is also the $\pi_{sol}$, therefore h($\pi_{i+1}$) = 0. By using Eq.~\eqref{aeq2:test}
and Eq.~\eqref{aeq3:test} together, we get $h^e(\pi_i)$ = 1. Therefore, the base step holds.
%
%
%

%
%\vspace{0.05in}
In the base case, we assume that after refinement step $R_i$, to be the best child, there is no unsupported causal link present in 
$\pi_{i+1}$ and a threat (if any) will be resolved by the planner immediately to make it a solution plan. 
%
If there is an unsupported causal link then there must be an existing action in $\pi_{i+1}$ to support it. 
In this case, the estimate of requirement of new actions is still be 0.

%
%
\noindent $\mathit{\bold{Hypothesis:}}$ We select an arbitrary partial plan $\pi_{i+1}$ and assume that Eq.~\eqref{eq2a:test} holds for it.
%

\noindent $\mathit{\bold{Proof \ Step:}}$
Here, we show that Eq.~\eqref{eq2a:test} holds for $\pi_i$ too.
%
%
%
\begin{eqnarray*}
		h^e(\pi_i) &=& cost(R_i)  +  h^e(\pi_{i+1}) \\						
						&=&  cost(R_i)  +  h(\pi_{i+1}) +  
										\sum_{\substack{\pi'~{\textit{from}} \
										\pi_{i+1} \rightsquigarrow \pi_{sol}}} \epsilon_{h(\pi')} \\
											&& \text{By the induction hypothesis.}
										\\ &=& h(\pi_{i})  +  \epsilon_{h(\pi_i)}
							  			 +  \sum_{\substack{\pi'~\textit{{from}} 
							  			 \ \pi_{i+1} \rightsquigarrow \pi_{sol}}} \epsilon_{h(\pi')} 
						  								~~\text{by Eq.~}\eqref{aeq3:test}.
%						  	\\ & & \hspace*{70pt} \bold{\because \ \ } \epsilon_{h(\pi_i)}  = 
%						  																	\big(cost(R_i) + h(\pi_{i+1})- h(\pi_{i})\big) 
							\\ &=& 	h(\pi_{i})  + \sum_{\substack{\pi'~\textit{{from}} \ \pi_{i} \rightsquigarrow 
							\pi_{sol}}} \epsilon_{h(\pi')}
\end{eqnarray*}
Therefore, the the relationship holds for the parent partial plan $\pi_i$ as well.
Thus, by induction for all partial plans $\pi$, our assumption is correct. $\hspace*{143pt}$ \tiny $\blacksquare$ 
\end{Proof}
%
%
%

==> gen-vis-time.tex <==
%
%
%
\begin{tabular}
%		
{
%
	@{}
				l
				>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad}  	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
				>{\small \tt} r
	@{}				
%
}
%
\toprule
%
	\multirow{2}{*}{Domain} & 
	\multicolumn{3}{c}{$h_{{add}}$} & 
	\multicolumn{3}{c}{\sc wef} & 
	\multicolumn{3}{c}{$h_{{add}}^r$} & 
	\multicolumn{3}{c}{\sc  wef} & 
	\multicolumn{3}{c}{$h_{{add}}$-\sc l } & 
	\multicolumn{3}{c}{$h_{{add}}\text{-\sc le}$} & 
	\multicolumn{3}{c}{\sc wef-l} & 
	\multicolumn{3}{c}{\sc wef-{le}} 
		\\ 	\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} \cmidrule(r){17-19}
			\cmidrule(r){20-22} \cmidrule(){23-25} 
	%
 	& 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} &
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} & 
 	\text{Gen} & 
 	\text{Vis} & 
 	\text{CPU} 
		\\ 		\cmidrule(r){1-1} \cmidrule(r){2-4} \cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(r){5-7}\cmidrule(lr){6-6}
				\cmidrule(lr){7-7}\cmidrule(r){8-10}\cmidrule(lr){9-9}\cmidrule(lr){10-10}\cmidrule(r){11-13} \cmidrule(lr){12-12}
				\cmidrule(lr){13-13}
				\cmidrule(r){14-16}\cmidrule(lr){15-15}\cmidrule(lr){16-16}\cmidrule(r){17-19}\cmidrule(lr){18-18}\cmidrule(lr){19-19}
				\cmidrule(r){20-22}
				\cmidrule(lr){21-21}\cmidrule(lr){22-22}\cmidrule(r){23-25}\cmidrule(lr){24-24}\cmidrule(l){25-25}
		%
		Gripper& 191 & 51 & 10 & 51 & 27 & 3.4 & 93 & 75 & 2.1 & 93 & 75 & 2.1
			 	& 38 & 17 & 1.4 & 37 & 17 & 2.3 & 37 & 17 & 2.3 &
			 	37 & 17 & 2.2 \\
		Rovers-3& 16 & 10 & 0.7 & 36 & 22 & 1.5 & 8 & 6 & 0.5 & 4 & 3 & 0.3
			 	& 19 & 7 & 0.9 & 19 & 9 & 10 & 19 & 9 & 10 & 19 & 9 & 10 \\ 
		Rovers -5& 70 & 32 & 3 & 67 & 38 & 5.2 & 96 & 51 & 12 & 34 & 26 & 11 &
			 	49 & 32 & 10 & 51 & 36 & 11 & 66 & 45 & 13 & 51 & 36 & 7 \\
		%
		%
\midrule
		%
		%
		\multirow{1}{*}{Domain} & 
		\multicolumn{3}{c}{$h_{{add}}$} & 
		\multicolumn{3}{c}{\sc wef} & 
		\multicolumn{3}{c}{$h_{{add}}^r$} & 
		\multicolumn{3}{c}{\sc wef} & 
		\multicolumn{3}{c}{$h_{{add}}^r$-\sc l}   & 
		\multicolumn{3}{c}{$h_{{add}}^r\text{-\sc le}$} & 
		\multicolumn{3}{c}{\sc wef-l}  &   							 
  		\multicolumn{3}{c}{\sc wef-{le}} 
			\\ 		\cmidrule(r){1-1} \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} 
					\cmidrule(r){14-16} \cmidrule(r){17-19} \cmidrule(r){20-22} \cmidrule(l){23-25} 
		%			 
		Logistics-1 & 89 & 9.5 & 100 & 0.4 & 0.2 & 0 & 64 & 12 & 64 & 1.9 & 0.6 & 46 &
				3 & 0.4 & 44 & 3 & 0.4 & 64 & 1.4 & 0.3 & 26 & 3 & 0.4 & 65 \\		 
		%
		%
		Elevator& 81 & 5.4 & 2 & 0.3 & 0.2 & 0 & 50 & 5 & 4 & 30 & 8 & 3 &
				12 & 1 & 0.6 & 12 & 1 & 0.6 & 12 & 1 & 0.6 &12 & 1 & 0.6  \\ 
		%
		Logistics-2 & 2 & 0.9 & 0.2 & 10 & 7 & 0.7 & 2.6 & 1.2 & 0.6 & 3 & 1.8 & 1 &
				0.6 & 0.2 & 0.1 & 0.6 & 0.2 & 0.1& 0.6 & 0.2 & 0.1& 0.6 & 0.2 & 0.1 \\
		%
		Zenotravel & 93 & 15 & 0.9 & 98 & 14 & 1 & 162 & 19 & 4 & 66 & 6 & 2&
				80 & 5 & 2.5 & 87 & 6.8 & 0.2 & 80 &4.5 & 2.9 & 88 & 7 & 2 \\				
%
\bottomrule			 
%
\end{tabular}
%
%

==> ipc-4.tex <==
\begin{tabular}{l @{\quad} >{\tt}c @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r @{\quad}>{\tt}r @{\quad}
>{\tt}r @{\quad} >{\tt}r @{\quad} >{\tt}r }%{|l|c|r| r r r |r| r r r |}
%
%
	\toprule
%
	\multirow{2}{*}{ \makecell{Domain \\ (IPC-4)} }  &
	%\multirow{2}{*}{ \normalfont Ins} &
	\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=r]{90}{\normalfont ~Ins}}} &
 	\multicolumn{4}{c}{$h_{{add}}^{{a}}$ with effort} & 		
	\multicolumn{4}{c}{$h_{{add}}$ with effort} 	\\ \cmidrule(r){3-6} \cmidrule{7-10}
	%
 	& & \multirow{1}{*}{\normalfont S} &
 	{\normalfont Gen} & {\normalfont Vis} & {\normalfont CPU} & \multirow{1}{*}{\normalfont S} &
 	{\normalfont Gen} & {\normalfont Vis} & {\normalfont CPU} \\ 
 	%
 	%
	%
	\cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){6-6}
		\cmidrule(r){7-10} \cmidrule(r){8-8} \cmidrule(r){9-10} \cmidrule(){10-10	}
	%
	%
	%	IPC-4
	Pipesworld-noTankage	&20	&{6}	&	8.3K	&	1.9K	&89		&5	&	8.1K	&1.4K	&109
	\\
	Pipesworld-tankage		&	20	& {3}	& {31K}	& {2.6K}	& {773}	&3	&	81K	&	6.9K	&2.1K
	\\
	Satellite	&	36	&	{24}	&	{96K}&	{4.1K}	&	{3.5K}	&2	&1.1K	&361	&2 
	\\ \bottomrule	
	%
	%
	%
\end{tabular}

==> problems-coverage-icaps-2016.tex <==
%
%
%
\begin{tabular}
%		
{ l | r r r r r r r r r r r r r r r r r}
%
\toprule
%
	\multirow{2}{*}{Domain} &
	\multicolumn{8}{c}{POCL Heuristics} &
	\multicolumn{5}{c}{Lazy} &
	\multicolumn{5}{c}{Eager}
	\\ \cmidrule{2-19}
	%
	 & 
	\multicolumn{1}{c}{$h_{{add}}$} & 
	\multicolumn{1}{c}{\sc wef} & 
	\multicolumn{1}{c}{$h_{{add}}^r$} & 
	\multicolumn{1}{c}{\sc  wef} & 
	\multicolumn{1}{c}{$h_{{add}}$-\sc l } & 
	\multicolumn{1}{c}{$h_{{add}}\text{-\sc le}$} & 
	\multicolumn{1}{c}{\sc wef-l} & 
	\multicolumn{1}{c}{\sc wef-{le}} &
	%
	\multicolumn{1}{c}{\sc ff} & 
	\multicolumn{1}{c}{\sc cea} &
	\multicolumn{1}{c}{\sc lmcut} &
	\multicolumn{1}{c}{\sc mhfs} &
	\multicolumn{1}{c}{\sc lama} &
	%
	\multicolumn{1}{c}{\sc ff} &
	\multicolumn{1}{c}{\sc cea} &
	\multicolumn{1}{c}{\sc lmcut} &
	\multicolumn{1}{c}{\sc mhfs} &
	\multicolumn{1}{c}{\sc lama}	
%
%
	\\ 	\midrule
%	
\bottomrule			 
%
\end{tabular}
%
%

==> solved-instances.tex <==
%
%
\begin{tabular}
%
{ 
	@{}
	l 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad}	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad}  	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{\quad} 	>{\small\tt} r 
				>{\small\tt} r 
	@{}
}
%
%
\toprule
	\multirow{2}{*}{Domain (n)} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}$} & 
	\multicolumn{2}{@{}c@{}}{\sc wef} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}^r$ } & 
	\multicolumn{2}{@{}c@{}}{\sc wef} & 
	\multicolumn{2}{@{}c@{}}{$h_{{add}}\text{-}\text{\sc l}$ } &
  	\multicolumn{2}{@{}c@{}}{$h_{\text{add}}\text{-}{\text{\sc le}}$} & 
  	\multicolumn{2}{@{}c@{}}{\sc wef-$\text{\sc l}$}  & 
  	\multicolumn{2}{@{}c@{}}{\sc wef-{\sc le}} 
  	%
	\\ 	\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
		\cmidrule(r){10-11} \cmidrule(r){12-13}
		\cmidrule(r){14-15} \cmidrule(){16-17} 
%
%
  & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} &
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} & 
  \normalfont{\sc s} & 
  \normalfont{\sc pl} 
 	\\ 	\cmidrule(r){1-1}  \cmidrule(r){2-3}  \cmidrule(r){3-3}  \cmidrule(r){4-5}  \cmidrule(r){5-5}  \cmidrule(r){6-7}  
 		\cmidrule(r){7-7} 	 \cmidrule(r){8-9}  \cmidrule(lr){9-9}  \cmidrule(r){10-11}  \cmidrule(r){11-11}  \cmidrule(r){12-13}
 		\cmidrule(r){13-13}  \cmidrule(r){14-15}  \cmidrule(r){15-15}  \cmidrule(r){16-17}  \cmidrule(l){17-17} 
  %  			
	Gripper (20) 	& 16 & 56 & 20 & 91 & 1 	& 15 & 1 	& 15 	& 20 & 68 & 20 & 68 & 20 & 68 & 20 & 68 \\
	Rovers-3 (20)	& 19 & 35 & 19 & 40 & 20 	& 37 & 20 	& 41 	& 20 & 37 & 20 & 37 & 20 & 37 & 20 & 37 \\
	Rovers-5 (40) 	& 28 & 48 & 31 & 65 & 32 	& 60 & 36 	& 102 	& 39 & 110 & 39 & 97 & 36 & 112 & 39 & 107 \\
  %
\bottomrule  
%			
\end{tabular}

==> solved-instances1.tex <==
%
%
\begin{tabular}
%
{
%	
	@{}
	l 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad}  	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{\quad} 	>{\small \tt} r 
				>{\small \tt} r 
	@{}
%
}
%
\toprule
%
%
	\multirow{2}{*}{Domain (n)} & 
	\multicolumn{2}{c}{$h_{{add}}$} & 
	\multicolumn{2}{c}{\sc wef} & 
	\multicolumn{2}{c}{$h_{{add}}^r$} & 
	\multicolumn{2}{c}{\sc wef}	& 
	\multicolumn{2}{c}{$h_{{add}}^r$-\sc l }  & 
  	\multicolumn{2}{c}{$h_{{add}}^r\text{-\sc  le}$} & 
  	\multicolumn{2}{c}{\sc wef-l} & 
  	\multicolumn{2}{c}{\sc wef-{\sc le}} 
		\\ 	\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
			\cmidrule(lr){10-11} \cmidrule(r){12-13}
			\cmidrule(r){14-15} \cmidrule(){16-17} 
%
	& 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} &
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
	\normalfont{\sc s} & 
	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} & 
 	\normalfont{\sc s} & 
 	\normalfont{\sc pl} 
 		\\ 	\cmidrule(r){1-1}  \cmidrule(r){2-3}  \cmidrule(r){3-3}  \cmidrule(r){4-5}  \cmidrule(r){5-5}  
 			\cmidrule(r){6-7}  \cmidrule(r){7-7}
 		 	\cmidrule(r){8-9}  \cmidrule(lr){9-9}  \cmidrule(r){10-11}  \cmidrule(r){11-11}  \cmidrule(r){12-13}
 		  	\cmidrule(r){13-13}  \cmidrule(r){14-15}  \cmidrule(r){15-15}  \cmidrule(r){16-17}  \cmidrule(l){17-17}
	%  			
	Logistics-1 (35) & {25} & 102 & 1 & 36 & 32 & 90 & 28 & 73 & 32 & 90 & 32 & 90 & 22 & 70 & 32 & 90 \\
	Elevator (150) & 148 & 54 & 14 & 9 & 150 & 55 & 58 & 29 & 150 & 55 & 150 & 55  & 150 & 55 & 150 & 55 \\
	Logistics-2 (40) & 36 & 77 & 12 & 53 & 36 & 63 & 34 & 63 & 40 & 63 & 40 & 65 & 40 & 63 & 40 & 65 \\
	Zenotravel (20) & 6 & 7 & 4 & 8 & 9 & 13 & 10 & 17 & 16 & 20 & 16 & 18 & 16 & 20 & 16 & 18 \\ 
	%
	\bottomrule  			
	%
\end{tabular}
%
%
